Dialogue Chain-of-Thought Distillation for Commonsense-aware Conversational Agents

Human-like chatbots necessitate the use of commonsense reasoning in order to effectively comprehend and respond to implicit information present within conversations. Achieving such coherence and informativeness in responses, however, is a non-trivial task. Even for large language models (LLMs), the task of identifying and aggregating key evidence within a single hop presents a substantial challenge. This complexity arises because such evidence is scattered across multiple turns in a conversation, thus necessitating integration over multiple hops. Hence, our focus is to facilitate such multi-hop reasoning over a dialogue context, namely dialogue chain-of-thought (CoT) reasoning. To this end, we propose a knowledge distillation framework that leverages LLMs as unreliable teachers and selectively distills consistent and helpful rationales via alignment filters. We further present DOCTOR, a DialOgue Chain-of-ThOught Reasoner that provides reliable CoT rationales for response generation. We conduct extensive experiments to show that enhancing dialogue agents with high-quality rationales from DOCTOR significantly improves the quality of their responses.

==> figure_latex/figure_comparison_with_human_curated.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=160mm]{figure/figure2.pdf}
    \caption{ Results of head-to-head comparison between dialogues from SODA, DailyDialog (Li et al., 2017),
and BlendedSkillTalk (Smith et al., 2020) via human judgments. The y-axis represents the number of samples
preferred by human judges. The differences in all of the categories except for the Context Dependence comparing
SODA and BlendedSkillTalk are statistically significant}\label{fig.comparison_with_human}
\end{figure*}

==> figure_latex/figure_diaoguecot.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=76mm]{figure/figure3_comparison.pdf}
    \caption{\textbf{A motivating example.} Comparison of dialogue Chain-of-Thought, single-hop reasoning (COMET), and vanilla Chain-of-Thought. }\label{fig.dialogue_cot}
\end{figure}

==> figure_latex/figure_human_eval_model.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=160mm]{figure/human_eval_dataset.png}
    \caption{Human evaluation on response generation model augmented with different knowledge sources.}
    \label{fig.human_eval_model}
\end{figure*}

==> figure_latex/figure_rg_quality.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figure/figure_rg_quality.png}
    \caption{Human evaluation results on the quality of responses generated from different sources of knowledge.}
    \label{fig:human_eval_rg}
\end{figure}

==> figure_latex/table_ablation.tex <==
\begin{table*}[!t]
\centering
\label{tab:ablation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcc}
\toprule
  &
  \multicolumn{4}{c}{DailyDialog} &
  \multicolumn{4}{c}{DREAM} &
  \multicolumn{4}{c}{MuTual} \\ \cmidrule(l){2-13} 
\textbf{Method} &
  B-1 &
  B-2 &
  B-4 &
  R-L &
  B-1 &
  B-2 &
  B-4 &
  R-L &
  B-1 &
  B-2 &
  B-4 &
  R-L  \\ \midrule
\textbf{COSMO} {[}3B{]} &
  18.21 &
  7.26 &
  2.05 &
  13.67 &
  17.07 &
  6.71 &
  1.8 &
  13.27 &
  16.87 &
  5.47 &
  1.11 &
  11.91 \\
+ COMET w/ S-BERT &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\
+ COMET w/ ComFact  &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\
+ DIALeCT  &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\ 
+ Reflect &
  17.60 &
  6.93 &
  1.97 &
  13.47 &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\
  + Ours &
  \textbf{18.78} &
  \textbf{7.72} &
  \textbf{2.23} &
  \textbf{14.18} &
  \textbf{17.69} &
  \textbf{6.90} &
  \textbf{1.82} &
  \textbf{13.36} &
  \textbf{17.10} &
   \textbf{5.78}&
  \textbf{1.16} &
  \textbf{12.62} \\
  
  \cmidrule(r){-}
\textbf{ChatGPT} {[}175B{]} &
  17.23 &
  7.16 &
  2.1 &
  14.72 &
  - &
  - &
  - &
  - &
  17.93 &
  7.01 &
  1.79 &
  14.77 \\
+ COMET w/ S-BERT &
  17.89 &
  7.28 &
  2.10 &
  14.35 &
  - &
  - &
  - &
  - &
  19.45 &
  7.82 &
  2.15 &
  \textbf{16.00} \\
+ COMET w/ ComFact  &
  18.23 & 
  7.5 &
  2.18 &
  14.35 &
  - &
  - &
  - &
  - &
  19.35 &
  7.72 &
  2.18 &
  15.50 \\ 
+ DIALeCT &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\ 
  + Reflect &
  17.27 &
  6.83 &
  1.98 &
  13.78 &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\
    + Self CoT &
  18.13 &
  7.23 &
  2.21 &
  12.61 &
  - &
  - &
  - &
  - &
  19.99 &
  7.33 &
  1.83 &
  13.67 \\+ Ours &
  \textbf{19.59} &
  \textbf{8.23} &
  \textbf{2.55} &
  \textbf{15.23} &
  - &
  - &
  - &
  - &
  \textbf{20.49} &
  \textbf{8.34}&
  \textbf{2.41} &
  15.97 \\
 \bottomrule
  
  
\end{tabular}%
}
\caption{Results on DailyDialog, DREAM, and MuTual compared with other knowledge sources.}
\label{tab:seen}
\end{table*}



==> figure_latex/table_example.tex <==

\begin{table}[t!]
\begin{center}\small
\renewcommand\thetable{2}
{
\begin{tabular}{l}
\hline
  \noalign{\hrule height0.8pt}
    \noalign{\smallskip}
    \textbf{Partner's personas:} \\
    I work out; I am a wrestler; ... \\\noalign{\smallskip}
    \textbf{Bot's personas:} \\
    I went for a run earlier; I eat a lot of beans for protein; ...\\\noalign{\smallskip}
    \hline
    % \noalign{\hrule height0.4pt}
    \noalign{\smallskip}
    \textbf{Dialogue history:} \\
     ...\\
     \emph{User}: Ok you guys should definitely be ready by then.\\
     Is your goal to win it or just run in it?\\\noalign{\smallskip}
     \hline
    % \noalign{\hrule height0.4pt}
    \noalign{\smallskip}
     \textbf{Semantic memory}:\\
     I am training for a walk or half marathon. \\\noalign{\smallskip}
     \textbf{Episodic memory}: My husband just convinced me to run\\
     my first. \underline{He has run 3 this year alone.} \\\noalign{\smallskip}
     \hline
     \noalign{\smallskip}
    \textbf{Response (w/ only semantic):}\\
    \emph{Agent}: Oh, I didn't think of that. I should definitely\\
    try to eat more beans. Do you have any good recipes?\\\noalign{\smallskip}
    \textbf{Response (\textit{Persona Replay}):}\\
    \emph{Agent}: Oh, my goal is just to finish it! \underline{My husband will} \\
    \underline{probably try to get in the top 10}, but for me it's\\ 
    just knowing that I did it the first time.\\
    \noalign{\smallskip}
  \hline
  \noalign{\hrule height0.8pt}
\end{tabular}
}
\end{center}
\caption{Responses predicted by our model and Poly-encoder (Semantic).}
\label{tab:example}
\end{table}

==> figure_latex/table_hyperparamter_tau.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|cccc|l}
    \toprule
    \tau   & B-1 & B-2 & B-4 & R-L & Relative size vs. DONUT \\
    \midrule
    0.9 & 18.75 & 7.73 & 2.26 & 14.69 & 1.1 \\
    0.95 (DONUT) & 19.61 & 8.44 & 2.69 & 15.63 & 1 \\
    1.0 & 19.58 & 8.34 & 2.6 & 15.52 & 0.47 \\
    1.05 & 19.15 & 8.13 & 2.51 & 15.19 & 0.19 \\
    
    \bottomrule 
    \end{tabular}
    \caption{Ablation study on different hyperparameters for $\tau$.}
    \label{tab.hyperparam_tau}
\end{table}

==> figure_latex/table_reasoning_order.tex <==
\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|cccc}
    \toprule
      \textbf{Reasoning Order}   & B-1 & B-2 & B-4 & R-L \\
      \midrule
       Forward (ours) & & & & \\
       Reverse & & & & \\
        Random & & & &\\ 
    
    \bottomrule 
    \end{tabular}
    \caption{Ablation study for different variations of reasoning orders.}
    \label{tab:reasoning_order}
\end{table}

==> figure_latex/table_seen_old.tex <==
\begin{table*}[!t]
\centering
\label{tab:seen_old}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc|cccc|cccc@{}}
\toprule
  &
  \multicolumn{4}{c}{DailyDialog} &
  \multicolumn{4}{c}{DREAM} &
  \multicolumn{4}{c}{MuTual} \\ \cmidrule(l){2-13} 
\textbf{Method} &
  B-1 &
  B-2 &
  B-4 &
  R-L &
  B-1 &
  B-2 &
  B-4 &
  R-L &
  B-1 &
  B-2 &
  B-4 &
  R-L  \\ \midrule
\textbf{COSMO} {[}3B{]} &
  20.04 &
  8.12 &
  2.38 &
  13.69 &
  20.98 &
  8.35 &
  2.28 &
  14.03 &
  17.63 &
  6.00 &
  1.30 &
  12.03 \\
% + COMET w/ S-BERT &
%   19.80 &
%   7.98 &
%   2.21 &
%   14.21 &
%   21.01  &
%   8.40  &
%   \textbf{2.31} &
%   13.88 &
%   17.75 &
%   6.29 &
%   1.57 &
%   \textbf{12.45} \\
+ COMET w/ ComFact  &
  19.54 &
  7.82 &
  2.25 &
  14.05 &
  20.90  &
  8.26  &
  2.17 &
  14.09 &
  17.56 &
  6.24 &
  1.37 &
  \textbf{12.41} \\
+ DIALeCT  &
  19.63 &
  8.05 &
  2.36 &
  14.31 &
  20.69 &
  8.18 &
  2.17 &
  13.82 &
  18.01 &
  6.35 &
  1.31 &
  12.23 \\ 
+ Reflect &
  19.44 &
  7.62 &
  2.11 &
  13.58 &
  18.23 &
  7.10 &
  1.91 &
  13.30 &
  \textbf{18.57} &
  6.13 &
  1.31 &
  12.01 \\
  + DOCTOR (Ours)&
  \textbf{20.43} &
  \textbf{8.54} &
  \textbf{2.63} &
  \textbf{14.68} &
  \textbf{21.26} &
  \textbf{8.65} &
  \textbf{2.46} &
  \textbf{14.26} &
  17.90 &
  \textbf{6.56} &
  \textbf{1.59} &
  12.35 \\
  
  \cmidrule(r){-}
\textbf{ChatGPT} {[}175B{]} &
  17.25 &
  7.18 &
  2.11 &
  14.72 &
  18.90 &
  7.81 &
  2.29 &
  14.86 &
  17.92 &
  7.03 &
  1.79 &
  14.83 \\
  % + COMET w/ S-BERT &
  % 17.89 &
  % 7.29 &
  % 2.11&
  % 14.36 &
  % 19.39 &
  % 7.65 &
  % 2.11 &
  % 14.12 &
  % 19.56 &
  % 7.87 &
  % 2.19 &
  % \textbf{16.05} \\
+ COMET w/ ComFact  &
  18.24 & 
  7.50 &
  2.19 &
  14.56 &
  20.09 &
  8.06 &
  2.33 &
  14.44 &
  19.32 &
  7.74&
  2.18 &
  15.46 \\ 
+ DIALeCT &
  16.61 &
  6.49 &
  1.82 &
  13.55 &
  18.00 &
  6.85&
  1.88 &
  13.16 &
  19.15 &
  7.67 &
  1.85 &
  \textbf{15.55} \\ 
  + Reflect &
  17.47 &
  6.98 &
  2.05 &
  13.80 &
  19.02 &
  7.35 &
  2.10 &
  13.37 &
  18.14 &
  6.87 &
  1.91 &
  14.27 \\
    + Self CoT &
  18.16 &
  7.24 &
  2.22 &
  12.62 &
  18.88 &
  7.13 &
  2.01 &
  12.17 &
  19.97 &
  7.32 &
  1.82 &
  13.71 \\
  + DOCTOR (Ours)&
  \textbf{19.61} &
  \textbf{8.44} &
  \textbf{2.69} &
  \textbf{15.63} &
  \textbf{21.20} &
  \textbf{8.71} &
  \textbf{2.56} &
  \textbf{14.93} &
  \textbf{20.19} &
  \textbf{8.35}&
  \textbf{2.52} &
\textbf{15.55}\\
 \bottomrule
  
  
\end{tabular}%
}
\caption{Automatic evaluation results on DailyDialog, DREAM, and MuTual using BLEU~\citep{papineni-etal-2002-bleu} and ROUGE~\citep{lin-2004-rouge}. We use B-1/2/4, and R-L to denote BLEU-1/2/4, and ROUGE-L for simplicity.  }
\label{tab:seen}
\end{table*}



==> figure_latex/table_unseen.tex <==

\begin{table}[!t]
\centering
\label{tab:unseen}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
 &
  \multicolumn{5}{c}{EmpatheticDialogues}
  \multicolumn{4}{c}{Reflect}
 \\ \cmidrule(l){2-9} 
\textbf{Method} &
  R-2 &
  R-L &
  B-2 &
  B-4 &
  R-2 &
  R-L &
  B-2 &
  B-4 \\ \midrule
\textbf{COSMO} {[}3B{]} &
 
  3.39 &
  13.27 &
  6.71 &
  1.8 &
  1.99 &
  11.91 &
  5.47 &
  1.11 \\
+ COMET w/ S-BERT &
  
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\
+ COMET w/ ComFact  &
  
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\
+ DIALeCT  &
 
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\ 
+ Reflect &
 
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\
  + DOCTOR (Ours)&
  
  3.45 &
  13.36 &
  6.9 &
  1.82 &
  2.29 &
  12.62 &
   5.78&
  1.16 \\
  \cmidrule(r){-}
\textbf{ChatGPT} {[}175B{]} &
 
  - &
  - &
  - &
  - &
  3.54 &
  14.77 &
  7.01 &
  1.79 \\
+ COMET w/ S-BERT &
 
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\
+ COMET w/ ComFact  &
 
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\
+ DIALeCT &
  
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\ 
  + Reflect &
 
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\
  + DOCTOR (Ours)&
 
  - &
  - &
  - &
  - &
  4.11 &
  15.97 &
  8.34 &
  2.41 \\
 \bottomrule
  
  
\end{tabular}
}
\caption{Automatic evaluation results on EmpatheticDialogues and Reflect. Note that we label these benchmarks as unseen since both our knowledge model and dialogue model are not trained on these corpora.}
\label{tab:unseen}
\end{table}
